Discrete Curvature Graph Information Bottleneck

Graph neural networks(GNNs) have been demonstrated to depend on whether the node effective information is sufficiently passing. Discrete curvature (Ricci curvature) is used to study graph connectivity and information propagation efficiency with a geometric perspective, and has been raised in recent years to explore the efficient message-passing structure of GNNs. However, most empirical studies are based on directly observed graph structures or heuristic topological assumptions and lack in-depth exploration of underlying optimal information transport structures for downstream tasks. We suggest that graph curvature optimization is more in-depth and essential than directly rewiring or learning for graph structure with richer message-passing characterization and better information transport interpretability. From both graph geometry and information theory perspectives, we propose the novel Discrete Curvature Graph Information Bottleneck (CurvGIB) framework to optimize the information transport structure and learn better node representations simultaneously. CurvGIB advances the Variational Information Bottleneck (VIB) principle for Ricci curvature optimization to learn the optimal information transport pattern for specific downstream tasks. The learned Ricci curvature is used to refine the optimal transport structure of the graph, and the node representation is fully and efficiently learned. Moreover, for the computational complexity of Ricci curvature differentiation, we combine Ricci flow and VIB to deduce a curvature optimization approximation to form a tractable IB objective function. Extensive experiments on various datasets demonstrate the superior effectiveness and interpretability of CurvGIB.

==> 9_checklist.tex <==
\section*{Reproducibility Checklist}
\begin{enumerate}
    \item This paper:
    \begin{itemize}
        \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. {\color{blue}[YES]}
        \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. {\color{blue}[YES]}
        \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. {\color{blue}[YES]}
    \end{itemize}

    \item Does this paper make theoretical contributions? {\color{blue}[YES]}
    If yes, please complete the list below.
    \begin{itemize}
        \item All assumptions and restrictions are stated clearly and formally. {\color{blue}[YES]}
        \item All novel claims are stated formally (e.g., in theorem statements). {\color{blue}[YES]}
        \item Proofs of all novel claims are included. {\color{blue}[YES]}
        \item Proof sketches or intuitions are given for complex and/or novel results. {\color{blue}[YES]}
        \item Appropriate citations to theoretical tools used are given. {\color{blue}[YES]}
        \item All theoretical claims are demonstrated empirically to hold. {\color{blue}[YES]}
        \item All experimental code used to eliminate or disprove claims is included. {\color{blue}[YES]}
    \end{itemize}

    \item Does this paper rely on one or more datasets? {\color{blue}[YES]}
    If yes, please complete the list below.
    \begin{itemize}
        \item A motivation is given for why the experiments are conducted on the selected datasets. {\color{blue}[YES]}
        \item All novel datasets introduced in this paper are included in a data appendix. {\color{gray}[NA]}
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. {\color{gray}[NA]}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. {\color{blue}[YES]}
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. {\color{blue}[YES]}
        \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. {\color{gray}[NA]}
    \end{itemize}

    \item Does this paper include computational experiments? {\color{blue}[YES]}
    If yes, please complete the list below.
    \begin{itemize}
        \item Any code required for pre-processing data is included in the appendix. {\color{blue}[YES]}
        \item All source code required for conducting and analyzing the experiments is included in a code appendix. {\color{blue}[YES]}
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. {\color{blue}[YES]}
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. {\color{blue}[YES]}
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. {\color{blue}[YES]}
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. {\color{blue}[YES]}
        \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. {\color{blue}[YES]}
        \item This paper states the number of algorithm runs used to compute each reported result. {\color{blue}[YES]}
        \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. {\color{blue}[YES]}
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). {\color{blue}[YES]}
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. {\color{blue}[YES]}
        \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. {\color{blue}[YES]}
    \end{itemize}
\end{enumerate}
